i-Rebalance: Personalized Vehicle Repositioning for Supply Demand Balance

Ride-hailing platforms have been facing the challenge of balancing demand and supply. Existing vehicle reposition techniques often treat drivers as homogeneous agents and relocate them deterministically, assuming compliance with the reposition. In this paper, we consider a more realistic and driver-centric scenario where drivers have unique cruising preferences and can decide whether to take the recommendation or not on their own. We propose i-Rebalance, a personalized vehicle reposition technique with deep reinforcement learning (DRL). i-Rebalance estimates drivers' decisions on accepting reposition recommendations through an on-field user study involving 99 real drivers. To optimize supply-demand balance and enhance preference satisfaction simultaneously, i-Rebalance has a sequential reposition strategy with dual DRL agents: Grid Agent to determine the reposition order of idle vehicles, and Vehicle Agent to provide personalized recommendations to each vehicle in the pre-defined order. This sequential learning strategy facilitates more effective policy training within a smaller action space compared to traditional joint-action methods. Evaluation of real-world trajectory data shows that i-Rebalance improves driver acceptance rate by 38.07% and total driver income by 9.97%.

==> Notation.tex <==
\section{Notation}
\begin{table}[h]
\centering
\begin{tabular}{|c|c|}
\hline
\textbf{Symbol} & \textbf{Meaning} \\
\hline
$i\in 0\dots 8$ & $3\times 3$ local index of grid\\
\hline
$g$ & global id of a grid\\
\hline 
$s\in S$ & state \\
\hline
$a\in A$ & action \\
\hline
$s_i^t$ & supply of gird $i$ at time $t$ \\
\hline
$d_i^t$ & demand of grid $i$ at time $t$ \\
\hline
$p_i^t$ & preference of driver to grid $i$ at time $t$\\
\hline
$r_B\in R_B$ & balance reward \\ 
\hline
$r_P\in R_P$ & preference reward \\ 
\hline
$r_R\in R_R$ & response reward \\ 
\hline
$\gamma_B$ & weight factor for $R_B$ \\ 
\hline
$\gamma_P$ & weight factor for $R_P$ \\ 
\hline
$\gamma_R$ & weight factor for $R_R$ \\
\hline
$\gamma$ & discount factor \\ 
\hline
$W_t$ & driver's state at time $t$\\
\hline
$L_t$ & location POI feature at time $t$\\
\hline
$T_t$ & location traffic feature at time $t$ \\
\hline
$V_t$ & location supply and demand features at time $t$\\
\hline
$P_{accept}$ & probability of accepting an instruction\\
\hline
$r$ & preference ranking of a certain grid\\
\hline
$m$ & expected income of a certain grid\\
\hline
$g_r$ & recommend grid \\
\hline
$\rho$ & recommend grid \\
\hline
\end{tabular}
\end{table}

==> RelatedWork.tex <==
\section{Related Work}


%- Traditional way to solve Unbalanced supply and demand (Non-DRL)

%- DRL based dispatching
%    - Centralised vs multi-agent
    
    
    
In this section, we discuss related vehicle repositioning techniques for balancing supply and demand, and techniques for modeling drivers' cruising preferences. 

% In this section,we summarize the state-of-the-art works in two fields which are related to our study: 1) reinforcement learning,and 2) driver preference modeling.

\subsection{Taxi reposition}
Taxi repositioning aims to relocate \TODO{idle vehicles} to demanding locations. 
%
With the help of massive taxi GPS trajectory data, existing works have been working on modeling and predicting travel demands of passengers and recommended profitable routes~\cite{qu2014cost}, spots~\cite{yuan2012t}, road clusters~\cite{wang2017taxirec} as well as social functional regions~\cite{kong2017time} to taxi drivers. 
% researchers can analyse and discover patterns to exploit, \cite{qu2014cost} build a profit function to recommend routes, \cite{yuan2012t} recommend demand hot spots, \cite{kong2017time} recommend according to time-location-relationship.
%
These works, however, recommended the top demanding locations to all the drivers, failing to consider competition between them. 
%
More advanced methods formulate taxi repositioning as an optimization problem, 
% such as combinatorial optimization or mixed integer programming, 
with the objectives to minimize the total idle cruising mileage of all vehicles~\cite{xie2018privatehunt,miao2016taxi,xu2018taxi} and the gap between supply and demand~\cite{miao2016taxi}.
%
These methods need to explicitly model the dynamic interactions between vehicles and ride demands with simplification such as assuming constant travel speed on the road networks, or constant arrival rate of ride requests, so they hardly adapt to the complex and highly dynamic environment.

% model demand and supply mathematically 

% but ignore the dynamic interactions between re-position actions and supply-demand balances. 

% However, this model-based method is limited by the pre-specified model and can not adapt to the complex dynamic environment.

% researchers build specific model of demand and supply, and dispatch taxis in a model-based way, the techniques varies, \cite{xie2018privatehunt} solved this problem with combinatorial optimization algorithm, \cite{miao2016taxi} used receding horizon control, \cite{xu2018taxi} exploit mixed-integer program. 

More recently, deep reinforcement learning has been used in vehicle repositioning problems~\cite{qin2022reinforcement}. 
%
By interacting with a simulated ride-hailing system, these model-free techniques are able to capture the interactions between repositioning actions and dynamic demands and can coordinate competing vehicles.   
%
Some works adopt a centralized strategy and train a single agent to learn reposition actions of all the vehicles~\cite{he2020spatio,oda2018movi,liu2020context}, but suffer from huge action search space. 
%
Others adopt a decentralized strategy and take each \TODO{idle vehicle} as an independent agent\cite{al2019deeppool,wen2017rebalancing}, but require training thousands of agents with high computational cost.
%
Further efforts have been made on simplifying the model, such as treating multiple agents in the same location as the same agent, that is, the agents share the same policy network~\cite{lin2018efficient}; averaging actions of agents in the same grids~\cite{li2019efficient}; training grid agent and vehicle agent with hierarchical reinforcement learning~\cite{jin2019coride}; and combining vehicle-location maximum matching optimization during DRL training~\cite{liu2021meta}.
%the agent is directly defined as a rasterized area, and the vehicles in the area will obey the scheduling action defined on the area [51].
% In these methods, agents can be map grids 

% The choice of agents in reinforcement learning varies, some prefer to choose map grids as agents \cite{yang2020multiagent}\cite{liu2021meta},  
% %
% \cite{jin2019coride} developed hierarchy between grids and solved reposition problem by dispatching fake orders, 
% %
% \cite{liu2021meta} introduce a two stage dispatch to make different actions for taxis. 
% The others model vehicles as agents\cite{liu2020context}\cite{lin2018efficient}\cite{wen2017rebalancing}, 
% %
% \cite{liu2020context} consider the context information while using a GNN to predict demand, 
% \cite{lin2018efficient} involve geographic context in a multiagent setting, \cite{lin2018efficient} adapted the problem to dynamic action space. These two choices have their own features, the grid agent can largely reduce agents' amount but is not specific when making dispatching decisions, the vehicle agent can be precise and specific but suffers from a big population and complex communication. 
%
These methods, however, assume that every driver unconditionally complies with the reposition recommendations.
In practice, however, drivers have their own preference on cruising routes~\cite{TrajGAIL,cGAIL} and they can reject repositioning recommendations in most ride-hailing platforms. Only \cite{xu2020recommender} takes driver acceptance into its reposition optimization model, but fails to consider drivers' personalized preferences. \TODO{\cite{he2020spatio} combines ride preference when dispatching under deep reinforcement learning framework, while ride preference is time invariant and homogeneous for different drivers.}

%
In contrast, i-Rebalance is the first work to consider drivers' personalized cruising preferences and the freedom to accept repositioning. 
%
We model driver preferences with a LSTM network to predict their next preferred location and conduct a user study to estimate the likelihood of acceptance. The two models are incorporated into our simulator and our reposition algorithms for personalized recommendations.

% Similar to these methods, our i-Rebalance re-positions vehicles with a deep reinforcement learning framework. But differently, we use two types of agents to interact with demands, i.e., grid agent to generate repositioning instructions and vehicle agent to respond instructions with personalized preferences.
% %
% To the best of our knowledge, this is the first work to consider drivers' unique preferences on cruising strategies and freedom to accept instructions. 

% Our work is the first to model the taxi reposition problem with a two-level agent design which takes advantage of both grid and vehicle agents. We are also the first to take into consideration of drivers' preference which makes our model more practical.  

% - traditional methods (5-6 sentences)

% - Reinforcement learning based method

% - Ours is different from these methods in 1) modeling drivers' preference 2) hierarchical reinforcement learning.

\begin{figure*}[!ht]
    \centering
    \includegraphics[width=0.9\textwidth]{Figure/framework.png}
    \vspace{-0.1in}
    \caption{Overview of i-Rebalance. \yan{
    i-Rebalance comprises two phases: 1) \textit{Driver Behavior Modeling} simulates realistic driver decision-making by predicting their cruising preferences and reposition acceptance probabilities. 2) \textit{Vehicle Repositioning with DRL} interacts with the simulator, employing two agents (Grid Agent and Vehicle Agent) to optimize repositioning. Grid Agent determines the sequence for repositioning based on supply-demand gaps and driver preferences within the grid. Vehicle Agent recommends destinations for each vehicle, focusing on individual preferences. Vehicle Agent receives rewards for supply-demand balance and preference satisfaction for each recommendation, while Grid Agent receives average rewards after all recommendations.}
    % i-Rebalance takes a city grid as an agent and observes supply and demand, as well as driver preference on the next cruising grids predicted by Cruising Preference Modeling. The grid agent makes repositioning recommendations to drivers. The simulator estimated whether a driver accepts the recommendation by Driver Decision Modeling. The agent receives rewards that measure the supply-demand balance, response rate to demands, and driver preference satisfaction.
    }
    \label{Fig:Overview}
\end{figure*}

\subsection{Cruising Preference Modeling}

Human trajectories have been used to understand their travel preferences in urban life~\cite{yang2020inferring}, route preference~\cite{zhao2016estimation}, and driving habits~\cite{xiao2020extracting}.
%
However, the preference of taxi or ride-hailing drivers on where to hunt for passengers did not get much attention.
% for taxis or ride-hailing drivers, although GPS on vehicles records their cruising trajectories, their preference 
%
Most existing works focus on mining the optimal strategy from trajectories, such as the optimal path that is most likely to get a passenger in the shortest time~\cite{rong2016rich,wang2015taxirec,yuan2012t}. 
%
Recently, \cite{IRLPreference,cGAIL,TrajGAIL,pan2020xgail} started to analyze the cruising strategies of taxi drivers and how the strategies affect income. %
They found that each driver has unique preferences on cruising routes, and the preferences tend to be stable over time. %Reverse reinforcement learning is adopted to predict the next cruising direction for each driver. 
%
This motivates us to recommend personalized repositioning to improve the drivers' satisfaction and acceptance.
However, their prediction networks in~\cite{cGAIL,TrajGAIL,pan2020xgail} cannot be used directly for vehicle repositioning as the networks are too complex to have an efficient prediction.

%
i-Rebalance needs to predict driver preference in every time step for each driver when interacting with the environment. For the efficiency of model training, the prediction model has to be lightweight. Therefore, we proposed a lightweight but effective LSTM prediction network.  
%and the DRL based reposition algorithm has to be trained  











% Driver preference modeling aims to learn where taxi drivers prefer to seek passengers when their taxis are vacant. In this field, plenty of research has been conducted by focusing on the dissection and prediction of inactive taxis’ trajectories. \cite{IRLPreference} analyzed history trajectory data by applying model-free Relative Entropy IRL based on Markov Decisiion Process and extracted taxi drivers' preference vector. Within the framework of Generative adversarial imitation learning, cGAIL \cite{cGAIL} learned taxi drivers' preference as policy function by training generator and discriminator in opposition to each other. cGAIL put forward the concept of conditional feature and succeeded in training different drivers in one unified model. Another solution is to modeling taxi drivers' decision process as variable length Markov decision processes (VLMDPs), based on which TrajGAIL \cite{TrajGAIL}  had a deep insight into a sequence of historical decisions.  


% Although all their frameworks have performed well in driver preference modeling, their complexity means these models are not suitable to be embedded in our dispatch model with heterogeneous drivers. Given that taxi trajectory data are human-generated spatial-temporal data,
%  plenty of works applied deep learning in the domain of traffic flow prediction, trajectory prediction and next location prediction.
 
 
%  Some works focused on statistical numbers of traffic flow. \cite{Revisit} built a Spatial-Temporal Dynamic Network, a combination of LSTM and CNN. They proposed flow gating mechanism and shifted attention mechanism to better predict the traffic flow between urban districts. \cite{conv-LSTM}used conv-LSTM to predict traffic flow, considering its special spatial-Temporal correlations. 
  
  
%   In the domain of small-scale trajectory prediction, \cite{socialLSTM} proposed an LSTM model which learns where pedestrians probably would go given the fact that human affect actions of people around. \cite{ma2019trafficpredict} proposed a LSTM-base algorithm to explore of movement patterns of different traffic-agents. By proposing a temporal pyramid network, \cite{liang2021temporal} solved a similar problem and achieved small displacement error.
  
  
  % Another related domain is next location prediction, which is also based on dissecting spatial-temporal data. The spatial context in 
 % \cite{liu2016predicting} is represented as Euclidean distance and the network is RNN-based. \cite{tang2019st} proposed HST-LSTM to predict user's movement in next minutes or hours but it defined location as functional zones rather than a geographical district.
 
 
 



